Categorical Generalization and Physical Structuralism

Category theory has become central to certain aspects of theoretical physics. Bain [Synthese, 190:1621--1635 (2013)] has recently argued that this has significance for ontic structural realism. We argue against this claim. In so doing, we uncover two pervasive forms of category-theoretic generalization. We call these `generalization by duality' and `generalization by categorifying physical processes'. We describe in detail how these arise, and explain their significance using detailed examples. We show that their significance is two-fold: the articulation of high-level physical concepts, and the generation of new models.

==> nCob <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Mar 06 17:48:23 GMT 2013
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3" x-max="11" y-min="1.5" y-max="4.5" auto-bounding="true">
%<ellipse fill-style= "none"
%	 p3= "(11,1.5)"
%	 p2= "(11,4.5)"
%	 p1= "(3,4.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(11,4.5)
\rput{0}(7,3){\psellipse[](0,0)(4,-1.5)}
\end{pspicture}


==> nCob2 <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Mar 06 17:48:13 GMT 2013
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3" x-max="11" y-min="1.5" y-max="11.5" auto-bounding="true">
%<ellipse fill-style= "none"
%	 p3= "(11,1.5)"
%	 p2= "(11,4.5)"
%	 p1= "(3,4.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(11,8.5)"
%	 p2= "(11,11.5)"
%	 p1= "(3,11.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3,10);(3,10);(3,3);(3,3)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11,10);(11,10);(11,3);(11,3)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(11,11.5)
\rput{0}(7,3){\psellipse[](0,0)(4,-1.5)}
\rput{0}(7,10){\psellipse[](0,0)(4,-1.5)}
\psline(3,10)(3,3)
\psline(11,10)(11,3)
\end{pspicture}


==> nCob3 <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Mar 06 17:48:01 GMT 2013
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.56" x-max="24.48" y-min="1.5" y-max="15" auto-bounding="true">
%<ellipse fill-style= "none"
%	 p3= "(11,1.5)"
%	 p2= "(11,4.5)"
%	 p1= "(3,4.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(17,12)"
%	 p2= "(17,15)"
%	 p1= "(9,15)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(24,1.5)"
%	 p2= "(24,4.5)"
%	 p1= "(16,4.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<pscurve fill-style= "none"
%	 closed= "false"
%	 curvature= "1;0.1;0"
%	 points= "(3,3);(3,3);(3,6);(8,10);(9,13);(9,13);
%	(4,17)"
%	 />
%<pscurve fill-style= "none"
%	 closed= "false"
%	 curvature= "1;0.1;0"
%	 points= "(24,3);(24,3);(24,6);(18,10);(17,13);(17,13);
%	(12,17)"
%	 />
%<pscurve fill-style= "none"
%	 closed= "false"
%	 curvature= "1;0.1;0"
%	 points= "(11,3);(11,3);(11,4);(12,7);(15,7);(16,4);
%	(16,3);(16,3)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(24.48,15)
\rput{0}(7,3){\psellipse[](0,0)(4,-1.5)}
\rput{0}(13,13.5){\psellipse[](0,0)(4,-1.5)}
\rput{0}(20,3){\psellipse[](0,0)(4,-1.5)}
\psecurve(3,3)(3,3)(3,6)(8,10)(9,13)(9,13)(4,17)
\psecurve(24,3)(24,3)(24,6)(18,10)(17,13)(17,13)(12,17)
\psecurve(11,3)(11,3)(11,4)(12,7)(15,7)(16,4)(16,3)(16,3)
\end{pspicture}


==> nCob4 <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Mar 07 10:35:59 GMT 2013
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3" x-max="22" y-min="1.5" y-max="4.5" auto-bounding="true">
%<ellipse fill-style= "none"
%	 p3= "(11,1.5)"
%	 p2= "(11,4.5)"
%	 p1= "(3,4.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(22,1.5)"
%	 p2= "(22,4.5)"
%	 p1= "(14,4.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(22,4.5)
\rput{0}(7,3){\psellipse[](0,0)(4,-1.5)}
\rput{0}(18,3){\psellipse[](0,0)(4,-1.5)}
\end{pspicture}


==> spek <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Apr 03 16:59:09 BST 2013
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16" y-min="0" y-max="4" auto-bounding="true">
%<parallelogram fill-style= "solid"
%	 p3= "(8,0)"
%	 fill-color= "#6699ff"
%	 p2= "(8,4)"
%	 p1= "(0,4)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(16,0)"
%	 p2= "(16,4)"
%	 p1= "(0,4)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4,4);(4,4);(4,0);(4,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8,4);(8,4);(8,0);(8,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12,4);(12,4);(12,0);(12,0)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16,4)
\newrgbcolor{userFillColour}{0.4 0.6 1}
\pspolygon[fillcolor=userFillColour,fillstyle=solid](0,4)(8,4)(8,0)(0,0)
\pspolygon[](0,4)(16,4)(16,0)(0,0)
\psline(4,4)(4,0)
\psline(8,4)(8,0)
\psline(12,4)(12,0)
\end{pspicture}

